Lottery Tickets with Nonzero Biases

The strong lottery ticket hypothesis holds the promise that pruning randomly initialized deep neural networks could offer a computationally efficient alternative to deep learning with stochastic gradient descent. Common parameter initialization schemes and existence proofs, however, are focused on networks with zero biases, thus foregoing the potential universal approximation property of pruning. To fill this gap, we extend multiple initialization schemes and existence proofs to nonzero biases, including explicit 'looks-linear' approaches for ReLU activation functions. These do not only enable truly orthogonal parameter initialization but also reduce potential pruning errors. In experiments on standard benchmark data, we further highlight the practical benefits of nonzero bias initialization schemes, and present theoretically inspired extensions for state-of-the-art strong lottery ticket pruning.

==> palettecolors.tex <==
% Color palettes inspired by works at the Metropolitan Museum of Art in New York, taken from https://github.com/BlakeRMills/MetBrewer
% Include via \usepackage{relative/path/to/palettecolors}
\RequirePackage{xcolor}
% Palette: Austria, #Colors: 7, Colorblind-friendly: False
\definecolor{austria(1)}{HTML}{a40000}
\definecolor{austria(2)}{HTML}{16317d}
\definecolor{austria(3)}{HTML}{007e2f}
\definecolor{austria(4)}{HTML}{ffcd12}
\definecolor{austria(5)}{HTML}{b86092}
\definecolor{austria(6)}{HTML}{721b3e}
\definecolor{austria(7)}{HTML}{00b7a7}
% Palette: Cassatt1, #Colors: 8, Colorblind-friendly: True
\definecolor{cassatt1(1)}{HTML}{b1615c}
\definecolor{cassatt1(2)}{HTML}{d88782}
\definecolor{cassatt1(3)}{HTML}{e3aba7}
\definecolor{cassatt1(4)}{HTML}{edd7d9}
\definecolor{cassatt1(5)}{HTML}{c9c9dd}
\definecolor{cassatt1(6)}{HTML}{9d9dc7}
\definecolor{cassatt1(7)}{HTML}{8282aa}
\definecolor{cassatt1(8)}{HTML}{5a5a83}
% Palette: Cassatt2, #Colors: 10, Colorblind-friendly: True
\definecolor{cassatt2(1)}{HTML}{2d223c}
\definecolor{cassatt2(2)}{HTML}{574571}
\definecolor{cassatt2(3)}{HTML}{90719f}
\definecolor{cassatt2(4)}{HTML}{b695bc}
\definecolor{cassatt2(5)}{HTML}{dec5da}
\definecolor{cassatt2(6)}{HTML}{c1d1aa}
\definecolor{cassatt2(7)}{HTML}{7fa074}
\definecolor{cassatt2(8)}{HTML}{466c4b}
\definecolor{cassatt2(9)}{HTML}{2c4b27}
\definecolor{cassatt2(10)}{HTML}{0e2810}
% Palette: Cross, #Colors: 9, Colorblind-friendly: False
\definecolor{cross(1)}{HTML}{c969a1}
\definecolor{cross(2)}{HTML}{ce4441}
\definecolor{cross(3)}{HTML}{ee8577}
\definecolor{cross(4)}{HTML}{eb7926}
\definecolor{cross(5)}{HTML}{ffbb44}
\definecolor{cross(6)}{HTML}{859b6c}
\definecolor{cross(7)}{HTML}{62929a}
\definecolor{cross(8)}{HTML}{004f63}
\definecolor{cross(9)}{HTML}{122451}
% Palette: Degas, #Colors: 7, Colorblind-friendly: False
\definecolor{degas(1)}{HTML}{591d06}
\definecolor{degas(2)}{HTML}{96410e}
\definecolor{degas(3)}{HTML}{e5a335}
\definecolor{degas(4)}{HTML}{556219}
\definecolor{degas(5)}{HTML}{418979}
\definecolor{degas(6)}{HTML}{2b614e}
\definecolor{degas(7)}{HTML}{053c29}
% Palette: Derain, #Colors: 7, Colorblind-friendly: True
\definecolor{derain(1)}{HTML}{efc86e}
\definecolor{derain(2)}{HTML}{97c684}
\definecolor{derain(3)}{HTML}{6f9969}
\definecolor{derain(4)}{HTML}{aab5d5}
\definecolor{derain(5)}{HTML}{808fe1}
\definecolor{derain(6)}{HTML}{5c66a8}
\definecolor{derain(7)}{HTML}{454a74}
% Palette: Egypt, #Colors: 4, Colorblind-friendly: True
\definecolor{egypt(1)}{HTML}{dd5129}
\definecolor{egypt(2)}{HTML}{0f7ba2}
\definecolor{egypt(3)}{HTML}{43b284}
\definecolor{egypt(4)}{HTML}{fab255}
% Palette: Gauguin, #Colors: 6, Colorblind-friendly: False
\definecolor{gauguin(1)}{HTML}{b04948}
\definecolor{gauguin(2)}{HTML}{811e18}
\definecolor{gauguin(3)}{HTML}{9e4013}
\definecolor{gauguin(4)}{HTML}{c88a2c}
\definecolor{gauguin(5)}{HTML}{4c6216}
\definecolor{gauguin(6)}{HTML}{1a472a}
% Palette: Greek, #Colors: 5, Colorblind-friendly: True
\definecolor{greek(1)}{HTML}{3c0d03}
\definecolor{greek(2)}{HTML}{8d1c06}
\definecolor{greek(3)}{HTML}{e67424}
\definecolor{greek(4)}{HTML}{ed9b49}
\definecolor{greek(5)}{HTML}{f5c34d}
% Palette: Hiroshige, #Colors: 10, Colorblind-friendly: True
\definecolor{hiroshige(1)}{HTML}{e76254}
\definecolor{hiroshige(2)}{HTML}{ef8a47}
\definecolor{hiroshige(3)}{HTML}{f7aa58}
\definecolor{hiroshige(4)}{HTML}{ffd06f}
\definecolor{hiroshige(5)}{HTML}{ffe6b7}
\definecolor{hiroshige(6)}{HTML}{aadce0}
\definecolor{hiroshige(7)}{HTML}{72bcd5}
\definecolor{hiroshige(8)}{HTML}{528fad}
\definecolor{hiroshige(9)}{HTML}{376795}
\definecolor{hiroshige(10)}{HTML}{1e466e}
% Palette: Hokusai1, #Colors: 7, Colorblind-friendly: False
\definecolor{hokusai1(1)}{HTML}{6d2f20}
\definecolor{hokusai1(2)}{HTML}{b75347}
\definecolor{hokusai1(3)}{HTML}{df7e66}
\definecolor{hokusai1(4)}{HTML}{e09351}
\definecolor{hokusai1(5)}{HTML}{edc775}
\definecolor{hokusai1(6)}{HTML}{94b594}
\definecolor{hokusai1(7)}{HTML}{224b5e}
% Palette: Hokusai2, #Colors: 6, Colorblind-friendly: True
\definecolor{hokusai2(1)}{HTML}{abc9c8}
\definecolor{hokusai2(2)}{HTML}{72aeb6}
\definecolor{hokusai2(3)}{HTML}{4692b0}
\definecolor{hokusai2(4)}{HTML}{2f70a1}
\definecolor{hokusai2(5)}{HTML}{134b73}
\definecolor{hokusai2(6)}{HTML}{0a3351}
% Palette: Hokusai3, #Colors: 6, Colorblind-friendly: True
\definecolor{hokusai3(1)}{HTML}{d8d97a}
\definecolor{hokusai3(2)}{HTML}{95c36e}
\definecolor{hokusai3(3)}{HTML}{74c8c3}
\definecolor{hokusai3(4)}{HTML}{5a97c1}
\definecolor{hokusai3(5)}{HTML}{295384}
\definecolor{hokusai3(6)}{HTML}{0a2e57}
% Palette: Homer1, #Colors: 8, Colorblind-friendly: False
\definecolor{homer1(1)}{HTML}{551f00}
\definecolor{homer1(2)}{HTML}{a62f00}
\definecolor{homer1(3)}{HTML}{df7700}
\definecolor{homer1(4)}{HTML}{f5b642}
\definecolor{homer1(5)}{HTML}{fff179}
\definecolor{homer1(6)}{HTML}{c3f4f6}
\definecolor{homer1(7)}{HTML}{6ad5e8}
\definecolor{homer1(8)}{HTML}{32b2da}
% Palette: Homer2, #Colors: 7, Colorblind-friendly: False
\definecolor{homer2(1)}{HTML}{bf3626}
\definecolor{homer2(2)}{HTML}{e9724c}
\definecolor{homer2(3)}{HTML}{e9851d}
\definecolor{homer2(4)}{HTML}{f9c53b}
\definecolor{homer2(5)}{HTML}{aeac4c}
\definecolor{homer2(6)}{HTML}{788f33}
\definecolor{homer2(7)}{HTML}{165d43}
% Palette: Ingres, #Colors: 8, Colorblind-friendly: True
\definecolor{ingres(1)}{HTML}{041d2c}
\definecolor{ingres(2)}{HTML}{06314e}
\definecolor{ingres(3)}{HTML}{18527e}
\definecolor{ingres(4)}{HTML}{2e77ab}
\definecolor{ingres(5)}{HTML}{d1b252}
\definecolor{ingres(6)}{HTML}{a97f2f}
\definecolor{ingres(7)}{HTML}{7e5522}
\definecolor{ingres(8)}{HTML}{472c0b}
% Palette: Isfahan1, #Colors: 7, Colorblind-friendly: True
\definecolor{isfahan1(1)}{HTML}{4e3910}
\definecolor{isfahan1(2)}{HTML}{845d29}
\definecolor{isfahan1(3)}{HTML}{d8c29d}
\definecolor{isfahan1(4)}{HTML}{4fb6ca}
\definecolor{isfahan1(5)}{HTML}{178f92}
\definecolor{isfahan1(6)}{HTML}{175f5d}
\definecolor{isfahan1(7)}{HTML}{1d1f54}
% Palette: Isfahan2, #Colors: 5, Colorblind-friendly: True
\definecolor{isfahan2(1)}{HTML}{d7aca1}
\definecolor{isfahan2(2)}{HTML}{ddc000}
\definecolor{isfahan2(3)}{HTML}{79ad41}
\definecolor{isfahan2(4)}{HTML}{34b6c6}
\definecolor{isfahan2(5)}{HTML}{4063a3}
% Palette: Juarez, #Colors: 6, Colorblind-friendly: False
\definecolor{juarez(1)}{HTML}{a82203}
\definecolor{juarez(2)}{HTML}{208cc0}
\definecolor{juarez(3)}{HTML}{f1af3a}
\definecolor{juarez(4)}{HTML}{cf5e4e}
\definecolor{juarez(5)}{HTML}{637b31}
\definecolor{juarez(6)}{HTML}{003967}
% Palette: Klimt, #Colors: 6, Colorblind-friendly: False
\definecolor{klimt(1)}{HTML}{df9ed4}
\definecolor{klimt(2)}{HTML}{c93f55}
\definecolor{klimt(3)}{HTML}{eacc62}
\definecolor{klimt(4)}{HTML}{469d76}
\definecolor{klimt(5)}{HTML}{3c4b99}
\definecolor{klimt(6)}{HTML}{924099}
% Palette: Lakota, #Colors: 6, Colorblind-friendly: False
\definecolor{lakota(1)}{HTML}{04a3bd}
\definecolor{lakota(2)}{HTML}{f0be3d}
\definecolor{lakota(3)}{HTML}{931e18}
\definecolor{lakota(4)}{HTML}{da7901}
\definecolor{lakota(5)}{HTML}{247d3f}
\definecolor{lakota(6)}{HTML}{20235b}
% Palette: Manet, #Colors: 11, Colorblind-friendly: False
\definecolor{manet(1)}{HTML}{3b2319}
\definecolor{manet(2)}{HTML}{80521c}
\definecolor{manet(3)}{HTML}{d29c44}
\definecolor{manet(4)}{HTML}{ebc174}
\definecolor{manet(5)}{HTML}{ede2cc}
\definecolor{manet(6)}{HTML}{7ec5f4}
\definecolor{manet(7)}{HTML}{4585b7}
\definecolor{manet(8)}{HTML}{225e92}
\definecolor{manet(9)}{HTML}{183571}
\definecolor{manet(10)}{HTML}{43429b}
\definecolor{manet(11)}{HTML}{5e65be}
% Palette: Monet, #Colors: 9, Colorblind-friendly: False
\definecolor{monet(1)}{HTML}{4e6d58}
\definecolor{monet(2)}{HTML}{749e89}
\definecolor{monet(3)}{HTML}{abccbe}
\definecolor{monet(4)}{HTML}{e3cacf}
\definecolor{monet(5)}{HTML}{c399a2}
\definecolor{monet(6)}{HTML}{9f6e71}
\definecolor{monet(7)}{HTML}{41507b}
\definecolor{monet(8)}{HTML}{7d87b2}
\definecolor{monet(9)}{HTML}{c2cae3}
% Palette: Moreau, #Colors: 7, Colorblind-friendly: False
\definecolor{moreau(1)}{HTML}{421600}
\definecolor{moreau(2)}{HTML}{792504}
\definecolor{moreau(3)}{HTML}{bc7524}
\definecolor{moreau(4)}{HTML}{8dadca}
\definecolor{moreau(5)}{HTML}{527baa}
\definecolor{moreau(6)}{HTML}{104839}
\definecolor{moreau(7)}{HTML}{082844}
% Palette: Morgenstern, #Colors: 7, Colorblind-friendly: True
\definecolor{morgenstern(1)}{HTML}{7c668c}
\definecolor{morgenstern(2)}{HTML}{b08ba5}
\definecolor{morgenstern(3)}{HTML}{dfbbc8}
\definecolor{morgenstern(4)}{HTML}{ffc680}
\definecolor{morgenstern(5)}{HTML}{ffb178}
\definecolor{morgenstern(6)}{HTML}{db8872}
\definecolor{morgenstern(7)}{HTML}{a56457}
% Palette: Nattier, #Colors: 7, Colorblind-friendly: False
\definecolor{nattier(1)}{HTML}{52271c}
\definecolor{nattier(2)}{HTML}{944839}
\definecolor{nattier(3)}{HTML}{c08e39}
\definecolor{nattier(4)}{HTML}{7f793c}
\definecolor{nattier(5)}{HTML}{565c33}
\definecolor{nattier(6)}{HTML}{184948}
\definecolor{nattier(7)}{HTML}{022a2a}
% Palette: Navajo, #Colors: 5, Colorblind-friendly: False
\definecolor{navajo(1)}{HTML}{660d20}
\definecolor{navajo(2)}{HTML}{e59a52}
\definecolor{navajo(3)}{HTML}{edce79}
\definecolor{navajo(4)}{HTML}{094568}
\definecolor{navajo(5)}{HTML}{e1c59a}
% Palette: NewKingdom, #Colors: 5, Colorblind-friendly: False
\definecolor{newkingdom(1)}{HTML}{e1846c}
\definecolor{newkingdom(2)}{HTML}{9eb4e0}
\definecolor{newkingdom(3)}{HTML}{e6bb9e}
\definecolor{newkingdom(4)}{HTML}{9c6849}
\definecolor{newkingdom(5)}{HTML}{735852}
% Palette: Nizami, #Colors: 8, Colorblind-friendly: False
\definecolor{nizami(1)}{HTML}{dd7867}
\definecolor{nizami(2)}{HTML}{b83326}
\definecolor{nizami(3)}{HTML}{c8570d}
\definecolor{nizami(4)}{HTML}{edb144}
\definecolor{nizami(5)}{HTML}{8cc8bc}
\definecolor{nizami(6)}{HTML}{7da7ea}
\definecolor{nizami(7)}{HTML}{5773c0}
\definecolor{nizami(8)}{HTML}{1d4497}
% Palette: OKeeffe1, #Colors: 11, Colorblind-friendly: True
\definecolor{okeeffe1(1)}{HTML}{6b200c}
\definecolor{okeeffe1(2)}{HTML}{973d21}
\definecolor{okeeffe1(3)}{HTML}{da6c42}
\definecolor{okeeffe1(4)}{HTML}{ee956a}
\definecolor{okeeffe1(5)}{HTML}{fbc2a9}
\definecolor{okeeffe1(6)}{HTML}{f6f2ee}
\definecolor{okeeffe1(7)}{HTML}{bad6f9}
\definecolor{okeeffe1(8)}{HTML}{7db0ea}
\definecolor{okeeffe1(9)}{HTML}{447fdd}
\definecolor{okeeffe1(10)}{HTML}{225bb2}
\definecolor{okeeffe1(11)}{HTML}{133e7e}
% Palette: OKeeffe2, #Colors: 7, Colorblind-friendly: True
\definecolor{okeeffe2(1)}{HTML}{fbe3c2}
\definecolor{okeeffe2(2)}{HTML}{f2c88f}
\definecolor{okeeffe2(3)}{HTML}{ecb27d}
\definecolor{okeeffe2(4)}{HTML}{e69c6b}
\definecolor{okeeffe2(5)}{HTML}{d37750}
\definecolor{okeeffe2(6)}{HTML}{b9563f}
\definecolor{okeeffe2(7)}{HTML}{92351e}
% Palette: Peru1, #Colors: 6, Colorblind-friendly: False
\definecolor{peru1(1)}{HTML}{b5361c}
\definecolor{peru1(2)}{HTML}{e35e28}
\definecolor{peru1(3)}{HTML}{1c9d7c}
\definecolor{peru1(4)}{HTML}{31c7ba}
\definecolor{peru1(5)}{HTML}{369cc9}
\definecolor{peru1(6)}{HTML}{3a507f}
% Palette: Peru2, #Colors: 7, Colorblind-friendly: False
\definecolor{peru2(1)}{HTML}{65150b}
\definecolor{peru2(2)}{HTML}{961f1f}
\definecolor{peru2(3)}{HTML}{c0431f}
\definecolor{peru2(4)}{HTML}{b36c06}
\definecolor{peru2(5)}{HTML}{f19425}
\definecolor{peru2(6)}{HTML}{c59349}
\definecolor{peru2(7)}{HTML}{533d14}
% Palette: Pillement, #Colors: 6, Colorblind-friendly: True
\definecolor{pillement(1)}{HTML}{a9845b}
\definecolor{pillement(2)}{HTML}{697852}
\definecolor{pillement(3)}{HTML}{738e8e}
\definecolor{pillement(4)}{HTML}{44636f}
\definecolor{pillement(5)}{HTML}{2b4655}
\definecolor{pillement(6)}{HTML}{0f252f}
% Palette: Pissaro, #Colors: 7, Colorblind-friendly: False
\definecolor{pissaro(1)}{HTML}{134130}
\definecolor{pissaro(2)}{HTML}{4c825d}
\definecolor{pissaro(3)}{HTML}{8cae9e}
\definecolor{pissaro(4)}{HTML}{8dc7dc}
\definecolor{pissaro(5)}{HTML}{508ca7}
\definecolor{pissaro(6)}{HTML}{1a5270}
\definecolor{pissaro(7)}{HTML}{0e2a4d}
% Palette: Redon, #Colors: 12, Colorblind-friendly: False
\definecolor{redon(1)}{HTML}{5b859e}
\definecolor{redon(2)}{HTML}{1e395f}
\definecolor{redon(3)}{HTML}{75884b}
\definecolor{redon(4)}{HTML}{1e5a46}
\definecolor{redon(5)}{HTML}{df8d71}
\definecolor{redon(6)}{HTML}{af4f2f}
\definecolor{redon(7)}{HTML}{d48f90}
\definecolor{redon(8)}{HTML}{732f30}
\definecolor{redon(9)}{HTML}{ab84a5}
\definecolor{redon(10)}{HTML}{59385c}
\definecolor{redon(11)}{HTML}{d8b847}
\definecolor{redon(12)}{HTML}{b38711}
% Palette: Renoir, #Colors: 12, Colorblind-friendly: False
\definecolor{renoir(1)}{HTML}{17154f}
\definecolor{renoir(2)}{HTML}{2f357c}
\definecolor{renoir(3)}{HTML}{6c5d9e}
\definecolor{renoir(4)}{HTML}{9d9cd5}
\definecolor{renoir(5)}{HTML}{b0799a}
\definecolor{renoir(6)}{HTML}{f6b3b0}
\definecolor{renoir(7)}{HTML}{e48171}
\definecolor{renoir(8)}{HTML}{bf3729}
\definecolor{renoir(9)}{HTML}{e69b00}
\definecolor{renoir(10)}{HTML}{f5bb50}
\definecolor{renoir(11)}{HTML}{ada43b}
\definecolor{renoir(12)}{HTML}{355828}
% Palette: Robert, #Colors: 6, Colorblind-friendly: False
\definecolor{robert(1)}{HTML}{11341a}
\definecolor{robert(2)}{HTML}{375624}
\definecolor{robert(3)}{HTML}{6ca4a0}
\definecolor{robert(4)}{HTML}{487a7c}
\definecolor{robert(5)}{HTML}{18505f}
\definecolor{robert(6)}{HTML}{062e3d}
% Palette: Signac, #Colors: 14, Colorblind-friendly: False
\definecolor{signac(1)}{HTML}{fbe183}
\definecolor{signac(2)}{HTML}{f4c40f}
\definecolor{signac(3)}{HTML}{fe9b00}
\definecolor{signac(4)}{HTML}{d8443c}
\definecolor{signac(5)}{HTML}{9b3441}
\definecolor{signac(6)}{HTML}{de597c}
\definecolor{signac(7)}{HTML}{e87b89}
\definecolor{signac(8)}{HTML}{e6a2a6}
\definecolor{signac(9)}{HTML}{aa7aa1}
\definecolor{signac(10)}{HTML}{9f5691}
\definecolor{signac(11)}{HTML}{633372}
\definecolor{signac(12)}{HTML}{1f6e9c}
\definecolor{signac(13)}{HTML}{2b9b81}
\definecolor{signac(14)}{HTML}{92c051}
% Palette: Stevens, #Colors: 6, Colorblind-friendly: False
\definecolor{stevens(1)}{HTML}{042e4e}
\definecolor{stevens(2)}{HTML}{307d7f}
\definecolor{stevens(3)}{HTML}{598c4c}
\definecolor{stevens(4)}{HTML}{ba5c3f}
\definecolor{stevens(5)}{HTML}{a13213}
\definecolor{stevens(6)}{HTML}{470c00}
% Palette: Tara, #Colors: 5, Colorblind-friendly: False
\definecolor{tara(1)}{HTML}{eab1c6}
\definecolor{tara(2)}{HTML}{d35e17}
\definecolor{tara(3)}{HTML}{e18a1f}
\definecolor{tara(4)}{HTML}{e9b109}
\definecolor{tara(5)}{HTML}{829d44}
% Palette: Thomas, #Colors: 8, Colorblind-friendly: False
\definecolor{thomas(1)}{HTML}{b24422}
\definecolor{thomas(2)}{HTML}{c44d76}
\definecolor{thomas(3)}{HTML}{4457a5}
\definecolor{thomas(4)}{HTML}{13315f}
\definecolor{thomas(5)}{HTML}{b1a1cc}
\definecolor{thomas(6)}{HTML}{59386c}
\definecolor{thomas(7)}{HTML}{447861}
\definecolor{thomas(8)}{HTML}{7caf5c}
% Palette: Tiepolo, #Colors: 8, Colorblind-friendly: False
\definecolor{tiepolo(1)}{HTML}{802417}
\definecolor{tiepolo(2)}{HTML}{c06636}
\definecolor{tiepolo(3)}{HTML}{ce9344}
\definecolor{tiepolo(4)}{HTML}{e8b960}
\definecolor{tiepolo(5)}{HTML}{646e3b}
\definecolor{tiepolo(6)}{HTML}{2b5851}
\definecolor{tiepolo(7)}{HTML}{508ea2}
\definecolor{tiepolo(8)}{HTML}{17486f}
% Palette: Troy, #Colors: 8, Colorblind-friendly: True
\definecolor{troy(1)}{HTML}{421401}
\definecolor{troy(2)}{HTML}{6c1d0e}
\definecolor{troy(3)}{HTML}{8b3a2b}
\definecolor{troy(4)}{HTML}{c27668}
\definecolor{troy(5)}{HTML}{7ba0b4}
\definecolor{troy(6)}{HTML}{44728c}
\definecolor{troy(7)}{HTML}{235070}
\definecolor{troy(8)}{HTML}{0a2d46}
% Palette: Tsimshian, #Colors: 7, Colorblind-friendly: False
\definecolor{tsimshian(1)}{HTML}{582310}
\definecolor{tsimshian(2)}{HTML}{aa361d}
\definecolor{tsimshian(3)}{HTML}{82c45f}
\definecolor{tsimshian(4)}{HTML}{318f49}
\definecolor{tsimshian(5)}{HTML}{0cb4bb}
\definecolor{tsimshian(6)}{HTML}{2673a3}
\definecolor{tsimshian(7)}{HTML}{473d7d}
% Palette: VanGogh1, #Colors: 7, Colorblind-friendly: False
\definecolor{vangogh1(1)}{HTML}{2c2d54}
\definecolor{vangogh1(2)}{HTML}{434475}
\definecolor{vangogh1(3)}{HTML}{6b6ca3}
\definecolor{vangogh1(4)}{HTML}{969bc7}
\definecolor{vangogh1(5)}{HTML}{87bcbd}
\definecolor{vangogh1(6)}{HTML}{89ab7c}
\definecolor{vangogh1(7)}{HTML}{6f9954}
% Palette: VanGogh2, #Colors: 8, Colorblind-friendly: False
\definecolor{vangogh2(1)}{HTML}{bd3106}
\definecolor{vangogh2(2)}{HTML}{d9700e}
\definecolor{vangogh2(3)}{HTML}{e9a00e}
\definecolor{vangogh2(4)}{HTML}{eebe04}
\definecolor{vangogh2(5)}{HTML}{5b7314}
\definecolor{vangogh2(6)}{HTML}{c3d6ce}
\definecolor{vangogh2(7)}{HTML}{89a6bb}
\definecolor{vangogh2(8)}{HTML}{454b87}
% Palette: VanGogh3, #Colors: 8, Colorblind-friendly: True
\definecolor{vangogh3(1)}{HTML}{e7e5cc}
\definecolor{vangogh3(2)}{HTML}{c2d6a4}
\definecolor{vangogh3(3)}{HTML}{9cc184}
\definecolor{vangogh3(4)}{HTML}{669d62}
\definecolor{vangogh3(5)}{HTML}{447243}
\definecolor{vangogh3(6)}{HTML}{1f5b25}
\definecolor{vangogh3(7)}{HTML}{1e3d14}
\definecolor{vangogh3(8)}{HTML}{192813}
% Palette: Veronese, #Colors: 7, Colorblind-friendly: True
\definecolor{veronese(1)}{HTML}{67322e}
\definecolor{veronese(2)}{HTML}{99610a}
\definecolor{veronese(3)}{HTML}{c38f16}
\definecolor{veronese(4)}{HTML}{6e948c}
\definecolor{veronese(5)}{HTML}{2c6b67}
\definecolor{veronese(6)}{HTML}{175449}
\definecolor{veronese(7)}{HTML}{122c43}
% Palette: Wissing, #Colors: 5, Colorblind-friendly: False
\definecolor{wissing(1)}{HTML}{4b1d0d}
\definecolor{wissing(2)}{HTML}{7c291e}
\definecolor{wissing(3)}{HTML}{ba7233}
\definecolor{wissing(4)}{HTML}{3a4421}
\definecolor{wissing(5)}{HTML}{2d5380}


==> palettes.tex <==
% Color palettes inspired by works at the Metropolitan Museum of Art in New York, taken from https://github.com/BlakeRMills/MetBrewer
% Include via \usepackage{relative/path/to/palettes}
\RequirePackage{xcolor}
\RequirePackage{pgfplots}
\RequirePackage{palettecolors}
% Palette: Austria, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{austria}{austria(1),austria(2),austria(3),austria(4),austria(5),austria(6),austria(7)}
% Palette: Cassatt1, #Colors: 8, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{cassatt1}{cassatt1(1),cassatt1(2),cassatt1(3),cassatt1(4),cassatt1(5),cassatt1(6),cassatt1(7),cassatt1(8)}
% Palette: Cassatt2, #Colors: 10, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{cassatt2}{cassatt2(1),cassatt2(2),cassatt2(3),cassatt2(4),cassatt2(5),cassatt2(6),cassatt2(7),cassatt2(8),cassatt2(9),cassatt2(10)}
% Palette: Cross, #Colors: 9, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{cross}{cross(1),cross(2),cross(3),cross(4),cross(5),cross(6),cross(7),cross(8),cross(9)}
% Palette: Degas, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{degas}{degas(1),degas(2),degas(3),degas(4),degas(5),degas(6),degas(7)}
% Palette: Derain, #Colors: 7, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{derain}{derain(1),derain(2),derain(3),derain(4),derain(5),derain(6),derain(7)}
% Palette: Egypt, #Colors: 4, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{egypt}{egypt(1),egypt(2),egypt(3),egypt(4)}
% Palette: Gauguin, #Colors: 6, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{gauguin}{gauguin(1),gauguin(2),gauguin(3),gauguin(4),gauguin(5),gauguin(6)}
% Palette: Greek, #Colors: 5, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{greek}{greek(1),greek(2),greek(3),greek(4),greek(5)}
% Palette: Hiroshige, #Colors: 10, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{hiroshige}{hiroshige(1),hiroshige(2),hiroshige(3),hiroshige(4),hiroshige(5),hiroshige(6),hiroshige(7),hiroshige(8),hiroshige(9),hiroshige(10)}
% Palette: Hokusai1, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{hokusai1}{hokusai1(1),hokusai1(2),hokusai1(3),hokusai1(4),hokusai1(5),hokusai1(6),hokusai1(7)}
% Palette: Hokusai2, #Colors: 6, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{hokusai2}{hokusai2(1),hokusai2(2),hokusai2(3),hokusai2(4),hokusai2(5),hokusai2(6)}
% Palette: Hokusai3, #Colors: 6, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{hokusai3}{hokusai3(1),hokusai3(2),hokusai3(3),hokusai3(4),hokusai3(5),hokusai3(6)}
% Palette: Homer1, #Colors: 8, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{homer1}{homer1(1),homer1(2),homer1(3),homer1(4),homer1(5),homer1(6),homer1(7),homer1(8)}
% Palette: Homer2, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{homer2}{homer2(1),homer2(2),homer2(3),homer2(4),homer2(5),homer2(6),homer2(7)}
% Palette: Ingres, #Colors: 8, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{ingres}{ingres(1),ingres(2),ingres(3),ingres(4),ingres(5),ingres(6),ingres(7),ingres(8)}
% Palette: Isfahan1, #Colors: 7, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{isfahan1}{isfahan1(1),isfahan1(2),isfahan1(3),isfahan1(4),isfahan1(5),isfahan1(6),isfahan1(7)}
% Palette: Isfahan2, #Colors: 5, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{isfahan2}{isfahan2(1),isfahan2(2),isfahan2(3),isfahan2(4),isfahan2(5)}
% Palette: Juarez, #Colors: 6, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{juarez}{juarez(1),juarez(2),juarez(3),juarez(4),juarez(5),juarez(6)}
% Palette: Klimt, #Colors: 6, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{klimt}{klimt(1),klimt(2),klimt(3),klimt(4),klimt(5),klimt(6)}
% Palette: Lakota, #Colors: 6, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{lakota}{lakota(1),lakota(2),lakota(3),lakota(4),lakota(5),lakota(6)}
% Palette: Manet, #Colors: 11, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{manet}{manet(1),manet(2),manet(3),manet(4),manet(5),manet(6),manet(7),manet(8),manet(9),manet(10),manet(11)}
% Palette: Monet, #Colors: 9, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{monet}{monet(1),monet(2),monet(3),monet(4),monet(5),monet(6),monet(7),monet(8),monet(9)}
% Palette: Moreau, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{moreau}{moreau(1),moreau(2),moreau(3),moreau(4),moreau(5),moreau(6),moreau(7)}
% Palette: Morgenstern, #Colors: 7, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{morgenstern}{morgenstern(1),morgenstern(2),morgenstern(3),morgenstern(4),morgenstern(5),morgenstern(6),morgenstern(7)}
% Palette: Nattier, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{nattier}{nattier(1),nattier(2),nattier(3),nattier(4),nattier(5),nattier(6),nattier(7)}
% Palette: Navajo, #Colors: 5, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{navajo}{navajo(1),navajo(2),navajo(3),navajo(4),navajo(5)}
% Palette: NewKingdom, #Colors: 5, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{newkingdom}{newkingdom(1),newkingdom(2),newkingdom(3),newkingdom(4),newkingdom(5)}
% Palette: Nizami, #Colors: 8, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{nizami}{nizami(1),nizami(2),nizami(3),nizami(4),nizami(5),nizami(6),nizami(7),nizami(8)}
% Palette: OKeeffe1, #Colors: 11, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{okeeffe1}{okeeffe1(1),okeeffe1(2),okeeffe1(3),okeeffe1(4),okeeffe1(5),okeeffe1(6),okeeffe1(7),okeeffe1(8),okeeffe1(9),okeeffe1(10),okeeffe1(11)}
% Palette: OKeeffe2, #Colors: 7, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{okeeffe2}{okeeffe2(1),okeeffe2(2),okeeffe2(3),okeeffe2(4),okeeffe2(5),okeeffe2(6),okeeffe2(7)}
% Palette: Peru1, #Colors: 6, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{peru1}{peru1(1),peru1(2),peru1(3),peru1(4),peru1(5),peru1(6)}
% Palette: Peru2, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{peru2}{peru2(1),peru2(2),peru2(3),peru2(4),peru2(5),peru2(6),peru2(7)}
% Palette: Pillement, #Colors: 6, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{pillement}{pillement(1),pillement(2),pillement(3),pillement(4),pillement(5),pillement(6)}
% Palette: Pissaro, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{pissaro}{pissaro(1),pissaro(2),pissaro(3),pissaro(4),pissaro(5),pissaro(6),pissaro(7)}
% Palette: Redon, #Colors: 12, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{redon}{redon(1),redon(2),redon(3),redon(4),redon(5),redon(6),redon(7),redon(8),redon(9),redon(10),redon(11),redon(12)}
% Palette: Renoir, #Colors: 12, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{renoir}{renoir(1),renoir(2),renoir(3),renoir(4),renoir(5),renoir(6),renoir(7),renoir(8),renoir(9),renoir(10),renoir(11),renoir(12)}
% Palette: Robert, #Colors: 6, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{robert}{robert(1),robert(2),robert(3),robert(4),robert(5),robert(6)}
% Palette: Signac, #Colors: 14, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{signac}{signac(1),signac(2),signac(3),signac(4),signac(5),signac(6),signac(7),signac(8),signac(9),signac(10),signac(11),signac(12),signac(13),signac(14)}
% Palette: Stevens, #Colors: 6, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{stevens}{stevens(1),stevens(2),stevens(3),stevens(4),stevens(5),stevens(6)}
% Palette: Tara, #Colors: 5, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{tara}{tara(1),tara(2),tara(3),tara(4),tara(5)}
% Palette: Thomas, #Colors: 8, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{thomas}{thomas(1),thomas(2),thomas(3),thomas(4),thomas(5),thomas(6),thomas(7),thomas(8)}
% Palette: Tiepolo, #Colors: 8, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{tiepolo}{tiepolo(1),tiepolo(2),tiepolo(3),tiepolo(4),tiepolo(5),tiepolo(6),tiepolo(7),tiepolo(8)}
% Palette: Troy, #Colors: 8, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{troy}{troy(1),troy(2),troy(3),troy(4),troy(5),troy(6),troy(7),troy(8)}
% Palette: Tsimshian, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{tsimshian}{tsimshian(1),tsimshian(2),tsimshian(3),tsimshian(4),tsimshian(5),tsimshian(6),tsimshian(7)}
% Palette: VanGogh1, #Colors: 7, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{vangogh1}{vangogh1(1),vangogh1(2),vangogh1(3),vangogh1(4),vangogh1(5),vangogh1(6),vangogh1(7)}
% Palette: VanGogh2, #Colors: 8, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{vangogh2}{vangogh2(1),vangogh2(2),vangogh2(3),vangogh2(4),vangogh2(5),vangogh2(6),vangogh2(7),vangogh2(8)}
% Palette: VanGogh3, #Colors: 8, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{vangogh3}{vangogh3(1),vangogh3(2),vangogh3(3),vangogh3(4),vangogh3(5),vangogh3(6),vangogh3(7),vangogh3(8)}
% Palette: Veronese, #Colors: 7, Colorblind-friendly: True
\pgfplotscreateplotcyclelist{veronese}{veronese(1),veronese(2),veronese(3),veronese(4),veronese(5),veronese(6),veronese(7)}
% Palette: Wissing, #Colors: 5, Colorblind-friendly: False
\pgfplotscreateplotcyclelist{wissing}{wissing(1),wissing(2),wissing(3),wissing(4),wissing(5)}

